On-Orbit Operations Simulator for Workload Measurement during Telerobotic Training

Training for telerobotic systems often makes heavy use of simulated platforms, which ensure safe operation during the learning process. Outer space is one domain in which such a simulated training platform would be useful, as On-Orbit Operations (O3) can be costly, inefficient, or even dangerous if not performed properly. In this paper, we present a new telerobotic training simulator for the Canadarm2 on the International Space Station (ISS), which is able to modulate workload through the addition of confounding factors such as latency, obstacles, and time pressure. In addition, multimodal physiological data is collected from subjects as they perform a task from the simulator under these different conditions. As most current workload measures are subjective, we analyse objective measures from the simulator and EEG data that can provide a reliable measure. ANOVA of task data revealed which simulator-based performance measures could predict the presence of latency and time pressure. Furthermore, EEG classification using a Riemannian classifier and Leave-One-Subject-Out cross-validation showed promising classification performance and allowed for comparison of different channel configurations and preprocessing methods. Additionally, Riemannian distance and beta power of EEG data were investigated as potential cross-trial and continuous workload measures.

==> CollisionsTable.tex <==
\begin{table}[]
\begin{tabular}{|c|cccccccc|}
\hline
Sub                         & \multicolumn{1}{c|}{RM \textgreater O1} & \multicolumn{1}{c|}{RM \textgreater O2} & \multicolumn{1}{c|}{RM \textgreater O3} & \multicolumn{1}{c|}{C2 \textgreater ISS} & \multicolumn{1}{c|}{C2 \textgreater O1} & \multicolumn{1}{c|}{C2 \textgreater O2} & \multicolumn{1}{c|}{C2 \textgreater O3} & Total                    \\ \hline
1                           & 11                                      & 2                                       & 1                                       & 8                                        & 1                                       & 2                                       & 0                                       & 25                       \\ \cline{1-1}
2                           & 9                                       & 0                                       & 0                                       & 2                                        & 0                                       & 1                                       & 0                                       & 12                       \\ \cline{1-1}
3                           & 0                                       & 0                                       & 0                                       & 0                                        & 0                                       & 0                                       & 0                                       & 0                        \\ \cline{1-1}
4                           & 9                                       & 0                                       & 0                                       & 0                                        & 0                                       & 0                                       & 0                                       & 9                        \\ \cline{1-1}
5                           & 10                                      & 5                                       & 4                                       & 1                                        & 0                                       & 3                                       & 2                                       & 25                       \\ \cline{1-1}
6                           & 4                                       & 0                                       & 0                                       & 3                                        & 0                                       & 0                                       & 0                                       & 7                        \\ \cline{1-1}
7                           & 6                                       & 2                                       & 0                                       & 7                                        & 0                                       & 1                                       & 0                                       & 16                       \\ \cline{1-1}
8                           & 0                                       & 3                                       & 5                                       & 0                                        & 0                                       & 0                                       & 0                                       & 8                        \\ \cline{1-1}
9                           & 2                                       & 0                                       & 0                                       & 1                                        & 0                                       & 2                                       & 0                                       & 5                        \\ \cline{1-1}
10                          & 4                                       & 1                                       & 1                                       & 7                                        & 0                                       & 3                                       & 0                                       & 16                       \\ \hline
\multicolumn{1}{|l|}{Total} & \multicolumn{1}{l}{55}                  & \multicolumn{1}{l}{13}                  & \multicolumn{1}{l}{11}                  & \multicolumn{1}{l}{29}                   & \multicolumn{1}{l}{1}                   & \multicolumn{1}{l}{12}                  & \multicolumn{1}{l}{2}                   & \multicolumn{1}{l|}{123} \\ \hline
\end{tabular}
\end{table}

==> SubjectResultsTable.tex <==
%($^{\circ}$)

\begin{table*}[t]
\caption{The mean, best, and worst performance measures for each of the 10 subjects. In this table, G and D represent the grappling and docking phases of the experiment, respectively. t, Dist, and Ang represent the time taken to achieve that phase, and the distance and angle between the end-effector's actual and ideal positions for each phase. FScore is the final score for a particular run. All time values are measures in seconds, while distances are measured in meters and angles are measured in degrees ($^{\circ}$).}
\label{tab:perf_measures}
\centering
\begin{tabular}{|c|c|cccccccccc|}
\hline
Sub                 & P.M.  & \multicolumn{1}{c|}{Gt} & \multicolumn{1}{c|}{GDist} & \multicolumn{1}{c|}{GAng} & \multicolumn{1}{c|}{GScore} & \multicolumn{1}{c|}{Dt} & \multicolumn{1}{c|}{DDist} & \multicolumn{1}{c|}{DAng} & \multicolumn{1}{c|}{DScore} & \multicolumn{1}{c|}{Dt-Gt} & FScore \\ \hline
\multirow{3}{*}{1}  & Mean  & 92.4                    & 0.478                      & 57.1                      & 254                         & 326                     & 0.595                      & 77.41                     & 208                         & 226                        & 15.1     \\ \cline{2-2}
                    & Best  & 35.2                    & 0.245                      & 32.1                      & 371                         & 158                     & 0.182                      & 43.36                     & 458                         & 105                        & 452    \\ \cline{2-2}
                    & Worst & 283                     & 0.764                      & 78.7                      & 0                           & 480                     & 1.393                      & 144.5                     & 0                           & 480                        & -580   \\ \hline
\multirow{3}{*}{2}  & Mean  & 46.2                    & 0.405                      & 50.0                      & 304                         & 225                     & 0.384                      & 56.69                     & 362                         & 179                        & 681    \\ \cline{2-2}
                    & Best  & 28.2                    & 0.219                      & 30.2                      & 222                         & 150                     & 0.104                      & 10.00                     & 823                         & 114                        & 1113   \\ \cline{2-2}
                    & Worst & 72.2                    & 0.768                      & 74.6                      & 424                         & 309                     & 1.027                      & 142.0                     & 0                           & 267                        & 223    \\ \hline
\multirow{3}{*}{3}  & Mean  & 101                     & 0.262                      & 39.7                      & 428                         & 201                     & 0.222                      & 45.3                      & 427                         & 99.8                       & 959    \\ \cline{2-2}
                    & Best  & 80.6                    & 0.044                      & 31.9                      & 824                         & 143                     & 0.135                      & 24.0                      & 535                         & 60.6                       & 1441   \\ \cline{2-2}
                    & Worst & 145                     & 0.643                      & 57.0                      & 272                         & 266                     & 0.367                      & 66.8                      & 310                         & 135                        & 689    \\ \hline
\multirow{3}{*}{4}  & Mean  & 32.0                    & 0.643                      & 69.6                      & 209                         & 151                     & 1.06                       & 78.9                      & 166                         & 119                        & 482    \\ \cline{2-2}
                    & Best  & 23.0                    & 0.290                      & 62.7                      & 325                         & 110                     & 0.292                      & 24.0                      & 351                         & 47.1                       & 691    \\ \cline{2-2}
                    & Worst & 68.8                    & 0.929                      & 89.2                      & 161                         & 338                     & 1.52                       & 125                       & 64                          & 142                        & 93     \\ \hline
\multirow{3}{*}{5}  & Mean  & 66.9                    & 0.670                      & 73.1                      & 203                         & 254                     & 0.97                       & 61.9                      & 176                         & 187                        & 377    \\ \cline{2-2}
                    & Best  & 33.2                    & 0.327                      & 61.6                      & 298                         & 149                     & 0.291                      & 46.5                      & 322                         & 103                        & 754    \\ \cline{2-2}
                    & Worst & 190                     & 0.948                      & 111                       & 138                         & 480                     & 1.49                       & 139                       & 0                           & 372                        & -125   \\ \hline
\multirow{3}{*}{6}  & Mean  & 45.9                    & 0.403                      & 82.3                      & 285                         & 169                     & 0.398                      & 70.9                      & 278                         & 107                        & 698    \\ \cline{2-2}
                    & Best  & 17.34                   & 0.14                       & 66.0                      & 481                         & 81.4                    & 0.105                      & 49.5                      & 579                         & 61.6                       & 1138   \\ \cline{2-2}
                    & Worst & 251.7                   & 0.789                      & 162                       & 162                         & 480                     & 1.258                      & 104                       & 0                           & 245                        & -113   \\ \hline
\multirow{3}{*}{7}  & Mean  & 85.4                    & 0.640                      & 72.4                      & 227                         & 295                     & 0.934                      & 74.49                     & 177                         & 209                        & 306    \\ \cline{2-2}
                    & Best  & 30.2                    & 0.183                      & 37.2                      & 459                         & 165                     & 0.229                      & 19.43                     & 508                         & 119                        & 792    \\ \cline{2-2}
                    & Worst & 177                     & 0.950                      & 114                       & 149                         & 480                     & 1.523                      & 135                       & 0                           & 364                        & -6     \\ \hline
\multirow{3}{*}{8}  & Mean  & 44.7                    & 0.554                      & 81.1                      & 221                         & 351                     & 0.969                      & 59.6                      & 142                         & 306                        & 226    \\ \cline{2-2}
                    & Best  & 34.2                    & 0.340                      & 62.2                      & 301                         & 185                     & 0.397                      & 26.28                     & 320                         & 141                        & 591    \\ \cline{2-2}
                    & Worst & 55.9                    & 0.815                      & 105                       & 176                         & 480                     & 1.494                      & 125                       & 0                           & 437                        & -194   \\ \hline
\multirow{3}{*}{9}  & Mean  & 46.7                    & 0.606                      & 65.8                      & 220                         & 180                     & 0.746                      & 66.4                      & 262                         & 133                        & 566    \\ \cline{2-2}
                    & Best  & 23.7                    & 0.384                      & 56.9                      & 281                         & 116                     & 0.136                      & 47.4                      & 499                         & 92.4                       & 842    \\ \cline{2-2}
                    & Worst & 191                     & 0.860                      & 82.2                      & 178                         & 398                     & 1.43                       & 141                       & 111                         & 222                        & 317    \\ \hline
\multirow{3}{*}{10} & Mean  & 84.2                    & 0.638                      & 78.4                      & 198                         & 304                     & 0.800                      & 61.6                      & 105                         & 225                        & 161    \\ \cline{2-2}
                    & Best  & 29.7                    & 0.460                      & 65.6                      & 249                         & 154                     & 0.405                      & 50.1                      & 270                         & 93.1                       & 568    \\ \cline{2-2}
                    & Worst & 255                     & 0.945                      & 101                       & 164                         & 480                     & 1.19                       & 80.6                      & 0                           & 425                        & -190   \\ \hline
\end{tabular}
\end{table*}

==> SubjectResultsTable2.tex <==

\begin{table*}[t]
\caption{The mean performance measures for each of the 10 subjects. In this table, G and D represent the grappling and docking phases of the experiment, respectively. t, Dist, and Ang represent the time taken to achieve that phase, and the distance and angle between the end-effector's actual and ideal positions for each phase. Coll is the total number of collisions throughout testing for a given subject. FScore is the final score for a particular run. All time values are measures in seconds, while distances are measured in meters and angles are measured in degrees ($^{\circ}$).}
\label{tab:perf_measures}
\centering
\begin{tabular}{|c|ccccccccclc|}
\hline
Sub & \multicolumn{1}{c|}{Gt} & \multicolumn{1}{c|}{GDist} & \multicolumn{1}{c|}{GAng} & \multicolumn{1}{c|}{GScore} & \multicolumn{1}{c|}{Dt} & \multicolumn{1}{c|}{DDist} & \multicolumn{1}{c|}{DAng} & \multicolumn{1}{c|}{DScore} & \multicolumn{1}{c|}{Dt-Gt} & \multicolumn{1}{l|}{Coll} & FScore \\ \hline
1   & 92.4                    & 0.478                      & 57.1                      & 254                         & 326                     & 0.595                      & 77.41                     & 208                         & 226                        & 25                        & 15     \\ \cline{1-1}
2   & 46.2                    & 0.405                      & 50.0                      & 304                         & 225                     & 0.384                      & 56.69                     & 362                         & 179                        & 12                        & 681    \\ \cline{1-1}
3   & 101                     & 0.262                      & 39.7                      & 428                         & 201                     & 0.222                      & 45.3                      & 427                         & 99.8                       & 0                         & 959    \\ \cline{1-1}
4   & 32.0                    & 0.643                      & 69.6                      & 209                         & 151                     & 1.06                       & 78.9                      & 166                         & 119                        & 9                         & 482    \\ \cline{1-1}
5   & 66.9                    & 0.670                      & 73.1                      & 203                         & 254                     & 0.97                       & 61.9                      & 176                         & 187                        & 25                        & 377    \\ \cline{1-1}
6   & 45.9                    & 0.403                      & 82.3                      & 285                         & 169                     & 0.398                      & 70.9                      & 278                         & 107                        & 7                         & 698    \\ \cline{1-1}
7   & 85.4                    & 0.640                      & 72.4                      & 227                         & 295                     & 0.934                      & 74.49                     & 177                         & 209                        & 16                        & 306    \\ \cline{1-1}
8   & 44.7                    & 0.554                      & 81.1                      & 221                         & 351                     & 0.969                      & 59.6                      & 142                         & 306                        & 8                         & 226    \\ \cline{1-1}
9   & 46.7                    & 0.606                      & 65.8                      & 220                         & 180                     & 0.746                      & 66.4                      & 262                         & 133                        & 5                         & 566    \\ \cline{1-1}
10  & 84.2                    & 0.638                      & 78.4                      & 198                         & 304                     & 0.800                      & 61.6                      & 105                         & 225                        & 16                        & 161    \\ \hline
\end{tabular}
\end{table*}

